Why Did This Model Forecast This Future? Closed-Form Temporal Saliency Towards Causal Explanations of Probabilistic Forecasts

Forecasting tasks surrounding the dynamics of low-level human behavior are of significance to multiple research domains. In such settings, methods for explaining specific forecasts can enable domain experts to gain insights into the predictive relationships between behaviors. In this work, we introduce and address the following question: given a probabilistic forecasting model how can we identify observed windows that the model considers salient when making its forecasts? We build upon a general definition of information-theoretic saliency grounded in human perception and extend it to forecasting settings by leveraging a crucial attribute of the domain: a single observation can result in multiple valid futures. We propose to express the saliency of an observed window in terms of the differential entropy of the resulting predicted future distribution. In contrast to existing methods that either require explicit training of the saliency mechanism or access to the internal states of the forecasting model, we obtain a closed-form solution for the saliency map for commonly used density functions in probabilistic forecasting. We empirically demonstrate how our framework can recover salient observed windows from head pose features for the sample task of speaking-turn forecasting using a synthesized conversation dataset.

==> scratch.tex <==

In such cases, we show that we can compute the differential entropy of the overall sequence by adding the entropy of the densities estimated at each timestep as follows. Considering two timesteps for simplicity, let us denote the random variables associated with the predictions as $Y_1$ and $Y_2$, and the sampled prediction from timestep $1$ as $\mybar{\bm{Y}}_1$. We then have
\begin{align}
    h(Y_1, Y_2) &= -\int\int p_{Y_1Y_2}(\bm{Y}_1, \bm{Y}_2)\log p_{Y_1Y_2}(\bm{Y}_1, \bm{Y}_2) d\bm{Y}_1d\bm{Y}_2\\
                &\approx -\int\int p_{Y_2|Y_1=\overline{\bm{Y}}_{\!\!1}}(\bm{Y}_2|\mybar{\bm{Y}}_1)p_{Y_1}(\bm{Y}_1)\log p_{Y_2|Y_1=\overline{\bm{Y}}_{\!\!1}}(\bm{Y}_2|\mybar{\bm{Y}}_1)p_{Y_1}(\bm{Y}_1) d\bm{Y}_1 d\bm{Y}_2\\
    \begin{split}
                &= -\int\int p_{Y_2|Y_1=\overline{\bm{Y}}_{\!\!1}}(\bm{Y}_2|\mybar{\bm{Y}}_1)p_{Y_1}(\bm{Y}_1)\log p_{Y_2|Y_1=\overline{\bm{Y}}_{\!\!1}}(\bm{Y}_2|\mybar{\bm{Y}}_1)d\bm{Y}_1 d\bm{Y}_2\\
                &\qquad\qquad\qquad -\int\int p_{Y_2|Y_1=\overline{\bm{Y}}_{\!\!1}}(\bm{Y}_2|\mybar{\bm{Y}}_1)p_{Y_1}(\bm{Y}_1)\log p_{Y_1}(\bm{Y}_1) d\bm{Y}_1 d\bm{Y}_2
    \end{split}
    \\[2ex]
    \begin{split}
                &= -\int p_{Y_1}(\bm{Y}_1)d\bm{Y}_1 \int p_{Y_2|Y_1=\overline{\bm{Y}}_{\!\!1}}(\bm{Y}_2|\mybar{\bm{Y}}_1)\log p_{Y_2|Y_1=\overline{\bm{Y}}_{\!\!1}}(\bm{Y}_2|\mybar{\bm{Y}}_1) d\bm{Y}_2\\
                &\qquad\qquad\qquad -\int p_{Y_2|Y_1=\overline{\bm{Y}}_{\!\!1}}(\bm{Y}_2|\mybar{\bm{Y}}_1)d\bm{Y}_2 \int p_{Y_1}(\bm{Y}_1)\log p_{Y_1}(\bm{Y}_1)d\bm{Y}_1
    \end{split}
    \\[2ex]
                &= - 1 \cdot  p_{Y_2|Y_1=\overline{\bm{Y}}_{\!\!1}}(\bm{Y}_2|\mybar{\bm{Y}}_1)\log p_{Y_2|Y_1=\overline{\bm{Y}}_{\!\!1}}(\bm{Y}_2|\mybar{\bm{Y}}_1) d\bm{Y}_2 - 1 \cdot p_{Y_1}(\bm{Y}_1)\log p_{Y_1}(\bm{Y}_1)d\bm{Y}_1\\
                &= h(Y2|Y1=\mybar{\bm{Y}}_1) + h(Y1)
\end{align}

% The forecasting of the low-level dynamics of human behavior constitutes an essential objective towards the development of machines with social intelligence, with implications for multiple fields including social psychology \cite{}, human-computer interaction \cite{}, and autonomous agent navigation \cite{}. While the focus of recent machine learning approaches in the research space has predominantly been on the \textit{how} questions\textemdash how can we develop methods for forecasting the future? \cite{}\textemdash domain experts concerned with gaining insight into human behavior are often interested in the \textit{what} and \textit{why} questions\textemdash  \textit{what} preceding behaviors forecast a certain social event of interest such as a speaker-turn change or interaction disengagement? and \textit{why} does a given model forecast a certain social future?  

% One broad strategy for enabling the asking of such \textit{what} and \textit{why} questions is to develop interpretable methods for time-series forecasting. However, recent methods for interpretable time-series forecasting mainly consider the point-forecasting problem \cite{}, which ignores a crucial attribute of the social behavior setting: a single sequence of observed behavior can result in multiple socially valid futures \citep[see][Sec.~2]{ramanSocialProcessesSelfSupervised2021}. For example, an interruption or window of overlapping speech may result in a change of speaker or a continuation with the same speaker \cite{duncanSignalsRulesTaking1972, heldnerPausesGapsOverlaps2010}, or a rotation of head may continue into a sweeping room-encompassing glance or fixation on a single person or object of attention \cite{mooreNonverbalCourtshipPatterns1985}.

%  In this paper, we focus on the developing an approach to assist the \textit{what} task. In this work, we introduce a novel research question within the task of social behavior forecasting: given a model that forecasts social futures, how can we identify sequences of preceding observed behavior that are salient for the model in making forecasts over a particular window? To address this question, we take an information theoretic perspective. We formalize temporal saliency in forecasting settings by building upon a simple core idea: the saliency of an observed sequence of behavior is directly related to the \textit{amount of information it contains about the future}. Concretely, taking inspiration from prior work on preattentive spatial saliency in images \cite{loogInformationTheoreticPreattentive2011}, we derive a closed-form expression for the associated saliency of an observed sequence by leveraging the entropy in the model's predicted distribution of future behaviors over a particular window.

% we leverage the variance in the social futures predicted by a model over a particular window to identify which preceding observed sequences of behavior were salient for the model in making the forecast. Concretely, we take an information theoretic perspective and formalize temporal saliency in behavior forecasting settings following a simple core idea: the saliency of an observed sequence of behavior is directly related to the amount of information it contains \textit{about the future}. Further, taking inspiration from prior work on preattentive spatial saliency in images \cite{loogInformationTheoreticPreattentive2011}, we derive a closed-form expression for the aforementioned temporal saliency.

% The immediate application of our proposed framework is in gaining insight into the observed behaviors upon which a model bases its specific forecasts. In cases where established social theories exist for how specific observed behaviors make certain future outcomes more likely than others, the framework can be used to sanity-check that the model considers those behaviors as salient towards its forecasts\textemdash  for instance, intonation \cite{keitel2015use}, gaze cues \cite{kalmaGazingTriadsPowerful1992}, and timing synchronization in speaker-listener speech \cite{levinsonTimingTurntakingIts2015} are predictive of subsequent turn changes. However, since both supporting and challenging arguments for such predictive relationships between social behaviors can be found in domain literature \citetext{\citealp[p.~5]{levinsonTimingTurntakingIts2015}; \citealp[p.~22]{kalmaGazingTriadsPowerful1992}}, a broader goal of our work here is to enable domain experts in forming new hypotheses surrounding associative and causal dependencies between social behaviors in a data-driven manner, using forecasting models trained on unconstrained in-the-wild behavior data. 


% \CR{Modeling the future using increasingly complex distributions has practical benefits when deployed for real-world applications. However, for the purpose of identifying salient predictive relationships between behaviors using our proposed framework, a simpler model forecasting a Gaussian distribution would work just as well, while also providing a closed-form expression. This follows from the entropy maximizing property of the Gaussian distribution: for a given covariance, the multivariate Gaussian distribution maximizes the entropy over all distributions \cite[see][Theorem~8.6.5]{coverElementsInformationTheory}. More formally, assuming a $d$-dimensional $Y$ and denoting the covariance of $Y|X=\bm{X}$ by $\bm{K}$, we have}
% \begin{equation}
%     h(Y|X=\bm{X}) \leq \frac{1}{2}\log[(2\pi e)^d\det(\bm{K})].
% \end{equation}
% \CR{This property implies that when considering two models that predict the same output covariance for an observation, the model assuming a unimodal Gaussian future density will produce the same saliency map as the model that assumes a more complex distribution such as a multimodal Gaussian mixture. This is because our framework only relies on relative changes in entropy (and the Gaussian distribution captures the maximum possible entropy for that covariance).}
